Localization on Snowflake Domains

The geometric features of the square and triadic Koch snowflake drums are compared using a position entropy defined on the grid points of the discretizations (pre-fractals) of the two domains. Weighted graphs using the geometric quantities are created and random walks on the two pre-fractals are performed. The aim is to understand if the existence of narrow channels in the domain may cause the `localization' of eigenfunctions.

==> bibliography.tex <==
\begin{thebibliography}{100}

\bibitem[At]{At} K. E. Atkinson,
\textit{An Introduction to Numerical Analysis}, 2nd edn., John
Wiley and Sons, New York (1989)

\bibitem [BeDe]{BeDe} R. J. Bell and P. Dean, \textit{Atomic vibrationsin vitreous
silica}, Disc. Faraday Soc. \textbf{50} (1970), 55-61


\bibitem[Be1]{Be1} M. V. Berry, \textit{Distribution of modes in fractal
resonators}, in: Structral Stability in Physics (W. G\"{u}ttinger,
and H. Eikemeier, eds.), Springer-Verlag, Berlin (1979), pp. 51-53

\bibitem[Be2]{Be2} M. V. Berry, \textit{Some geometric aspects of wave motion:
Wavefront dislocations, diffraction catatrophes, diffractals}, in:
Geometry of the Laplace Operator, Proc. Sympos. Pure Math., vol.
36, Amer. Math. Soc., Providence, R. I. (1980), pp. 13-38

\bibitem[BroCa]{BroCa} J. Brossard and R. Carmona, Can one hear
the dimension of a fractal?, \textit{Commun. Math. Phys.}
\textbf{104} (1986), 103-122

\bibitem[Ev]{Ev} L. C. Evans,
\textit{Partial Differential Equations}, Graduate Studies in
Mathematics, vol. 19, Amer. Math. Soc., Providence, R. I. (1998)

\bibitem [EveRRPS]{EveRRPS}  C. Even,  S. Russ,  V. Repain, P.
Pieranski and B. Sapoval, \textit{Localization in fractal drums:
An experimental study}, Phys. Rev. Lett. {\bf 83} (1999), 726-729


\bibitem[F]{F} K. J. Falconer,
\textit{Fractal Geometry: Mathematical Foundations and
Applications}, John Wiley and Sons, London (1990)

\bibitem[Ha]{Ha} M. J. W. Hall, \textit{Universal geometric approach
to uncertainty, entropy and information}, Phys. Rev. A \textbf{50}
(1999), 2602-2615

\bibitem[IK]{IK}  E. Isaacson and H. Keller,
\textit{Analysis of Numerical Methods}, John Wiley and Sons, New
York (1966)

\bibitem [L1]{L1} M. L. Lapidus, Fractal drum, inverse spectral
problems for elliptic operators and a partial resolution of the
Weyl--Berry conjecture, \textit{Trans. Amer. Math. Soc.}
\textbf{325} (1991), 465-529

\bibitem [L2]{L2} M. L. Lapidus, \textit{Spectral and fractal geometry:
 From the Weyl--Berry conjecture for the vibrations of fractal dums
 to the Riemann zeta-function}, in: Differential Equations and
 Mathematical Physics (C. Bennewitz, ed.), Proc. Fourth UAB
 Internat. Conf. (Birmingham, March 1990), Academic Press, New York,
 1992, pp. 151-182

\bibitem [L3]{L3} M. L. Lapidus, \textit{Vibrations of fractal drums,
the Riemann hypothesis, waves in fractal media, and the
Weyl--Berry conjecture}, in: Ordinary and Partial Differential
Equations (B. D. Sleeman and R. J. Jarvis, eds.), vol. IV, Proc.
Twelfth Internat. Conf. (Dundee, Scotland, UK, June 1992), Pitman
Research Notes in Math. Series, vol. 289, Longman Scientific and
Technical, London, 1993, pp. 126-209


\bibitem[LP]{LP} M. L. Lapidus and M. M. H. Pang,
\textit{Eigenfunctions of the Koch snowflake domain}, Commun.
Math. Phys. {\bf 172} (1995), 359-376


\bibitem[LNRG]{LNRG}  M. L. Lapidus, J. W. Neuberger,  R. J. Renka
and C. A. Griffith, \textit{Snowflake harmonics and computer
graphics: Numerical computation of spectra on fractal drums},
Internat. J. Bifurcation \& Chaos \textbf{6} (1996), 1185-1210


\bibitem[Sa1]{Sa1} B. Sapoval, \textit{Fractals}, Bernard Aumont, Aditech,
Paris (1990)

\bibitem[Sa2]{Sa2} B. Sapoval, \textit{Experimental observation of local modes in fractal
drums}, Physica D {\bf 38} (1989), 296-298

\bibitem [SG]{SG} B. Sapoval and T. Gobron, \textit{Vibrations of strongly irregular
or fractal resonators}, Phys. Rev. E {\bf 47} (1993), 3013-3024


\bibitem [SGM]{SGM}  B. Sapoval, T. Gobron and  A. Margolina, \textit{Vibrations of fractal
drums}, Phys. Rev. Lett. {\bf 67} (1991), 2974-2977


\bibitem [Si]{Si} I. Simonsen, \textit{Diffusion and networks: A powerful combination!},
Physica A {\bf 357} (2005), 317-330



\bibitem [SiErMaSn]{SiErMaSn} I. Simonsen, K. A. Eriksen, S.
Maslov and K. Sneppen, \textit{Diffusion on complex networks: A
way to probe their large-scale topological structures}, Physica A
{\bf 336} (2004), 163-173




\bibitem[Th]{Th} D. J. Thouless, \textit{Electrons in disordered
systems and the theory of localization}, Phys. Rep. \textbf{13}
(1974), 93-142

\bibitem [We]{We} F. Wegner, \textit{Bounds on the density of states in disordered systems},
Z. Phys. B \textbf{44} (1981), 9-15
\end{thebibliography}

